The Planted Matching Problem: Phase Transitions and Exact Results

We study the problem of recovering a planted matching in randomly weighted complete bipartite graphs $K_{n,n}$. For some unknown perfect matching $M^*$, the weight of an edge is drawn from one distribution $P$ if $e \in M^*$ and another distribution $Q$ if $e \notin M^*$. Our goal is to infer $M^*$, exactly or approximately, from the edge weights. In this paper we take $P=\exp(\lambda)$ and $Q=\exp(1/n)$, in which case the maximum-likelihood estimator of $M^*$ is the minimum-weight matching $M_{\text{min}}$. We obtain precise results on the overlap between $M^*$ and $M_{\text{min}}$, i.e., the fraction of edges they have in common. For $\lambda \ge 4$ we have almost perfect recovery, with overlap $1-o(1)$ with high probability. For $\lambda < 4$ the expected overlap is an explicit function $\alpha(\lambda) < 1$: we compute it by generalizing Aldous' celebrated proof of the $\zeta(2)$ conjecture for the un-planted model, using local weak convergence to relate $K_{n,n}$ to a type of weighted infinite tree, and then deriving a system of differential equations from a message-passing algorithm on this tree.

==> Sections/JointDef.tex <==
%\cris{Looking at this section (which is only about one page long) I feel that the general reader will have a hard time understanding why we need it or what it's for. Can you provide a sentence or two about that?}
%\mr{How about the following:
%``To use the local weak framework to study convergence of minimum matchings, we are going to append $\{0,1\}$ to the edges of planted networks in $\Gstar$.''
%Then we can start from second paragraph: 
%``Generally speaking, we can think of .... ''
%up to 
%``may not be a matching).''
%Next, we should add the first paragraph:
%``For a network $N$ we define $\mathcal{M}[N]$  ..... ''
%I also think the following sentence at the end of the second paragraph is redundant:
%``For a network $N$ we define $\mathcal{M}[N]$ .....''
%}
%\cris{Should $\m$ be $\M$ here? This may have been my mistake.}\mr{I use $\m$ as a fixed matching, and $\M$ when randomness is involved. I am ok if you want to combine them (it might be even better).}

%Consider a planted network $N = (G,\ell)$ where $G = (V,E,M)$.  A matching $\m$ on $N$ (not to be confused with the planted matching $\Mplanted$) is a subset of $E$  such that every vertex has exactly one incident edge in this subset. We can think of a matching as a function over the edges as well as the nodes: for every edge $e\in E$, we define $\m(e) = 1$ if $e$ is in the matching and $\m(e) = 0$ otherwise. As stated above, for every vertex $v\in V$, we define its partner $\m(v) = w$ if $e = \{v,w\}$ is a member of the matching. \cris{Some of this is redundant with Section $1$ or can be moved there.} \mr{Agree}
%%Note that the set of planted edges $M$ is always a matching. 

% THIS IS NOW MOVED TO OptMatch.tex
For a network $N$ we define $\mathcal{M}[N]$ as the set of all matchings on $N$. 
Now, a random matching on $N$ is a joint distribution of length of the edges and matchings on $N$ with marginal $\ell$. That is to say, $(\ell,\M)$ is a probability measure on $\rplus^E \times \mathcal{M}[N]$ with marginal $\ell$ on $\rplus^E$. 

\begin{remark}
Intuitively, the reader would probably interpret the phrase ``random matching'' as a measurable function from $\rplus^E \to \mathcal{M}[N]$. However, here we follow Aldous by using it to mean a distribution over both the lengths $\ell$ and the matching itself.
\end{remark}

% THIS IS NOW MOVED TO JointConv.tex
We can think of a matching $\M$ on $N$ as a mark function that assigns $0$ or $1$ to the edges of $N$. So, to use the framework of local weak convergence to study minimum matchings, we append $\{0,1\}$ to the edges of planted networks in $\Gstar$. In a slight abuse of terminology, we call $\widehat{N} = (G,\ell,\M)$ a planted network where $(\ell,\M):E \to \rplus \times \{0,1\}$, where $\ell$ is the weight function and $\M$ is a mark function (which may or may not be a matching). Then a random matching is a joint distribution on $(\ell,\M)$, where $\M$ ranges over $\mathcal{M}[N]$. 
%\mr{This is really important to include, since initially we treated $\m$ just as a mark function.}.

% we you use Gmadstar only once, in Involinvar.tex
All the definitions in Section~\ref{sec:gen_setup} extend naturally to this new setting. We use $\,\widehat{\textrm{hat}}\,$ to distinguish these two cases from each other e.g., $\Gmadstar$ denotes members of $\Gstar$ together with a mark function ranging over $\{0,1\}$.

Recall that $\Mnopt$ denotes the minimum matching on $(K_{n,n},\ell_n)$. Since the minimum matching is unique with probability $1$ in our model, we can think of $\Mnopt$ as a deterministic function of the edge lengths $\ell_n$. We are interested in the weak limit of $\widehat{\mu}_n = \Exp U(\widehat{N}_n) \in \mathcal{P}(\Gmadstar)$, where $\widehat{N}_n = (K_{n,n},(\ell_n,\Mnopt))$ and $U(\widehat{N}_n)$ is defined similarly to $U(N_n)$ in~\eqref{eq:local-uniform}. In other words, we now want to understand the limiting distribution of neighborhoods that include edge weights, the planted matching $M_n$, and the minimum matching $\Mnopt$---so that, for instance, we can compute the expectation of the overlap $(1/n) |M_n \cap \Mnopt|$.

Note that the uniform choice of root in the definition of $U(\widehat{N}_n)$ implies that $\widehat{N}_n$ is involution invariant. Moreover, as before every vertex in the planted model has the same distribution of neighborhoods, so we can take the root to be vertex $1$: that is, $\widehat{\mu}_n$ is the distribution of $[\widehat{N}_n(1)]$. 
%\mr{Also note that, by the symmetric structure of the planted model, 
Thus the averaged expected cost of $\Mnopt$ is
\begin{align}\label{eq:optmatfin}
\frac{1}{n} \,\E{\sum_{\Mnopt(e)= 1} \ell_n(e)} = \E{\ell_n(1,\Mnopt(1))}. 
\end{align}
where the expectation is over the randomness in the model, i.e., over the edge weights.

Since $\mu_n$ converges locally weakly to $\mu_\infty$, a natural guess would be that the weak limit of $\widehat{N}_n$ is a random matching on the planted PWIT. Moreover, since $\widehat{\mu}_n$ is involution invariant and involution invariance passes through the weak limit \cite[Section 5.2]{Aldous2004}, this random matching on the planted PWIT should be involution invariant. Hence, the goal is to show that the weak limit is the law of $[\widehat{N}_{\infty,\circ}]$ where $\widehat{N}_{\infty,\circ} = (T_\infty,(\ell_\infty,\Minfopt))$ and $(\ell_\infty,\Minfopt)$ is the minimum involution invariant random matching on the planted PWIT. That is to say, the weak limit is $\widehat{\mu}_\infty$ where $[\widehat{N}_{\infty,\circ}]\sim \widehat{\mu}_\infty$  and $\widehat{\mu}_\infty$ is involution invariant according to Definition \ref{def:spinvar}. %Let us first introduce the infinite involution invariant matching $\Minfopt$ and prove its optimality. 

\mr{You decided to remove the part related to the topological discussion?}
\cris{This was commented out (not deleted) from OptMatch.tex. I have put it in this .tex but still commented. I still don't see the necessity, but maybe I will after reading Appendix F.}\mr{Great, thanks! I am fine if you want to delete it.}

%\mr{Before proceeding any further, let us take care of some topological details. Let $\mathcal{G}_{*,\infty}\subset \Gstar$ denote the set of all possible realizations of planted PWIT. We can think of $\mathcal{G}_{*,\infty}$  as a subspace of $[0,\infty)^{E_{\infty}}$. The space $[0,\infty)^{E_{\infty}}$ is equipped with a natural topology (product topology, coordinate wise convergence) and a natural $\sigma$-algebra (product $\sigma$-algebra). This topology is finer than the topology of $\mathcal{G}_{*,\infty}$, and the Borel $\sigma$ algebra on $\mathcal{G}_{*,\infty}$ is a subset of the product $\sigma$-algebra on $[0,\infty)^{E_{\infty}}$. Hence, we can safely focus on $[0,\infty)^{E_{\infty}}$ using its natural topology and $\sigma$-algebra.} \mr{In my opinion we are precise enough. Defining the ordering on the edges in kind of overkill, but let me know if it is ambiguous. }

%Also, it is easy to see that open sets in  $\Gstar$ can be mapped to open sets in $[0,\infty)^{E_{\infty}}$. Hence, any measure that is defined over $[0,\infty)^{E_{\infty}}$
%	
%	Hence, any property that holds for $[0,\infty)^{E_{\infty}}$ with its natural topology, also holds for $\Gstar$ restricted to all possible realizations of PWIT. To be more specific, we are going to explicitly define the natural topology of $[0,\infty)^{E_{\infty}}$.
%
%Let us first assign labels to the edges of $E_{\infty}$. We label the edge $\{\bs{i},\bs{i}j\}$ with $\bs{i}j$. Now, for any two edge $\bs{i} = i_1i_2\cdots i_l$ and $\bs{j} = j_1j_2\cdots j_l$ we say $\bs{i} \precr \bs{j}$ if either $\sum i_s < \sum j_s$, or $\sum i_s = \sum j_s$ and $l<k$, or $\sum i_s = \sum j_s$, $l=k$ and there is a $t$ such that $i_s = j_s$ for all $s<t$ and $i_t < j_t$. Now, order the edges using this ordering:
%\begin{align*}
%0 \precr 1\precr 2 \precr 11 \precr 3 \precr 12 \precr 21 \precr 111 \precr 4 \precr \cdots
%\end{align*}
%Now, the natural topology on $[0,\infty)^{E_{\infty}}$ is the infinite product topology, and convergence in this topology means the coordinate-wise convergence of the edge weights.}



==> Sections/erlangdiff.tex <==
The moment generating function for an exponential random variable $Y$ with rate $\lambda$ is
\[
\expect[\e^{\mu Y}] = \frac{\lambda}{\lambda-\mu} \, . 
\]
Since $X_1$ and $X_2$ are independent, the exponential generating function for $X_1-X_2$ is
\begin{equation}
\label{eq:mgf-x1-x2}
\expect[\e^{\mu (X_1-X_2)}]
= \expect[\e^{\mu X_1}] \,\expect[\e^{-\mu X_2)}]
= \left( \frac{\lambda_1 \lambda_2}{(\lambda_1-\mu)(\lambda_2+\mu)} \right)^{\!t} \, ,
\end{equation}
By Markov's inequality
\[
\prob[X_1 > X_2] = \prob[\e^{\mu (X_1-X_2)} > 1] \le \expect[\e^{\mu (X_1-X_2)}] 
\]
for any $\mu > 0$. The right-hand side of~\eqref{eq:mgf-x1-x2} is minimized when $\mu = (\lambda_1-\lambda_2)/2$, giving the desired result.
